Audio Similarity is Unreliable as a Proxy for Audio Quality

Many audio processing tasks require perceptual assessment. However, the time and expense of obtaining ``gold standard'' human judgments limit the availability of such data. Most applications incorporate full reference or other similarity-based metrics (e.g. PESQ) that depend on a clean reference. Researchers have relied on such metrics to evaluate and compare various proposed methods, often concluding that small, measured differences imply one is more effective than another. This paper demonstrates several practical scenarios where similarity metrics fail to agree with human perception, because they: (1) vary with clean references; (2) rely on attributes that humans factor out when considering quality, and (3) are sensitive to imperceptible signal level differences. In those scenarios, we show that no-reference metrics do not suffer from such shortcomings and correlate better with human perception. We conclude therefore that similarity serves as an unreliable proxy for audio quality.

==> LaTeX/IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> LaTeX/tables/differences_scenario2.tex <==
\begin{table}[b!]
\vspace{0\baselineskip}
\centering
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c}
 \toprule
 \multirow{1}{*}{\bf Type} & \multirow{1}{*}{\bf Ref} 
 & \bf PESQ$\uparrow$ &\bf VISQOL$\uparrow$ &\bf DPAM$\downarrow$ &\bf CDPAM$\downarrow$ &\bf L1$\downarrow$ &\bf L2$\downarrow$ &\bf M.STFT$\downarrow$ & \bf SQAPP$\uparrow$ & \bf NISQA$\uparrow$  & \bf DNSMOS$\uparrow$  & \bf NORESQA$\downarrow$ \\
 \cmidrule(lr){1-13}
 
 {\bf \multirow{2}{*}{\bf Test Rec. 1}} 
  & Ref 1 & 1.81 & 3.321  & 1.789 & 0.128 & 747.192 & 9.004 & 0.101 & 3.708  &  3.800 & 3.640 & 10.793  \\
  & Ref 2 & 3.05 & 3.610 & 2.619 & 0.068 & 634.119 & 7.773 & 0.094 & 3.836 & 3.899 & 3.555 & 10.592  \\
  \hline
 {\bf \multirow{2}{*}{\bf Test Rec. 2}} 
  & Ref 1 & 1.889 & 4.492 & 1.717   & 0.039 & 270.98 & 3.032 & 0.072  & 4.017 & 4.10 & 3.518 & 10.899    \\
  & Ref 2 & 3.739 & 4.119 & 2.640  & 0.064 & 295.811 & 3.383 & 0.075 & 4.114 & 4.212 & 3.503 & 11.066   \\
 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{\textbf{Scenario 1}: Two test recordings are each compared with two clean quality reference recordings (but recorded under two environments). Similarity metrics show different similarities, whereas no-reference metrics (and subjective ratings) suggest that the two references are of equal quality.}

%Performance of similarity metrics, distance metrics and subjective ratings on two examples where we use same quality clean references (but recorded under two environments), and compare it to the same test recording. } 
\vspace{-0.2in}
\label{low_quality_sec4.2}
\end{table}

==> LaTeX/tables/griffin_lim.tex <==
\begin{table}[h!]
\vspace{0\baselineskip}
\centering
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multicolumn{10}{c}{\bf Objective Metrics} \\
 \cmidrule(lr){2-11} 
 &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS  \\
 \cmidrule(lr){1-11}
 {\bf Non-match. frame and hop sizes} \\
 {\bf itr 0} 
 &  &  &  &  &  &  &  &  &  &   \\
  {\bf itr 200} 
 &  &  &  &  &  &  &  &  &  &   \\
  {\bf itr 1000} 
 &  &  &  &  &  &  &  &  &  &   \\
 \hline
 {\bf Match. frame and hop sizes} \\ 
 {\bf itr 0} 
 &  &  &  &  &  &  &  &  &  &   \\
  {\bf itr 200} 
 &  &  &  &  &  &  &  &  &  &   \\
  {\bf itr 1000} 
 &  &  &  &  &  &  &  &  &  &   \\
 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{Griffin Lim scores}
\vspace{-0.2in}
\label{griffin_lim_scores}
\end{table}

==> LaTeX/tables/high_pass_filtering.tex <==
\begin{table}[t!]
\vspace{-2\baselineskip}
\centering
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multicolumn{11}{c}{\bf Objective Metrics} \\
 \cmidrule(lr){2-12} 
 &\bf PESQ$\uparrow$ &\bf VISQOL$\uparrow$ &\bf DPAM$\downarrow$ &\bf CDPAM$\downarrow$ &\bf L1$\downarrow$ &\bf L2$\downarrow$ &\bf M.STFT$\downarrow$ & \bf SQAPP$\uparrow$ & \bf NISQA$\uparrow$  & \bf DNSMOS$\uparrow$ & \bf NORESQA$\downarrow$  \\
 \cmidrule(lr){1-12}
 {\bf Clean reference} 
 & - & - & - & - & - & - & - & 4.11  & 4.06 & 3.47 & 9.342  \\
 {\bf Test Recording} 
 & 2.54 & 3.69 & 2.74 & 0.25 & 1226.62 & 11.60 & 0.16 & 4.03 & 4.16 & 3.56 & 9.619 \\
 {\bf Test+high-pass filter.} 
 & 2.84 & 3.10 & 2.57 & 0.14 & 896.18 & 6.92 & 0.23 & 4.01 & 4.01 & 3.53 &  10.097 \\
 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{\textbf{High-pass filtering}: Objective measures when high-pass filtering is applied on a test recording.}
\vspace{-0.2in}
\label{high_pass_filtering}
\end{table}

==> LaTeX/tables/maleVSfemale.tex <==
\begin{table}[b!]
\vspace{0\baselineskip}
\centering
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c}
 \toprule
 \multirow{1}{*}{\bf Type} & \multirow{1}{*}{\bf Ref} 
 %& \multicolumn{10}{c}{\bf DAPS Model~\cite{jin2017voco}} \\
%  \cmidrule(lr){2-11} 
 &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS \\
 \cmidrule(lr){1-12}
 
 {\bf \multirow{2}{*}{\bf DAPS}} 
  & Male & &  &  &  &  &  &  &  &  &  &   
  & Female & &  &  &  &  &  &  &  &  &  &   
  \hline
 {\bf \multirow{2}{*}{\bf VCTK}} 
  & Male & &  &  &  &  &  &  &  &  &  &  
  & Female & &  &  &  &  &  &  &  &  &  &    
 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{Male VS Female scores}
\vspace{-0.2in}
\label{maleVSfemale}
\end{table}

==> LaTeX/tables/modelDAPSvsmodelVCTK_repeat.tex <==



\section{Suppliers' production capabilities}

\setlength{\extrarowheight}{2pt}
\begin{longtable}{@{} ZZ | ZZ @{}}

%%% headers and footers:

\caption{Supplier facilities' production capabilities }
\hline
\textbf{Facility Name} & \textbf{Product} & 
\textbf{Facility Name} & \textbf{Product} \\
\hline
\endfirsthead

\multicolumn{4}{@{}l}{Table \thetable, cont'd}\\[1ex]
\hline
\textbf{Facility Name} & \textbf{Product} & 
\textbf{Facility Name} & \textbf{Product} \\
\hline
\endhead

\hline
\multicolumn{4}{r@{}}{\footnotesize cont'd on following page}\\
\endfoot

\hline
\endlastfoot

%%% Body of table

Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
Texttext texttextt exttextt & Wordswordswords wordswordswords & Texttext texttextt exttexttex exttexttex & Wordswordswords wordswordswords \\
\end{longtable}


==> LaTeX/tables/ref_deg_both_noise_added.tex <==
\begin{figure}[t!]
\vspace{-0\baselineskip}
\centering
\setlength{\w}{0.32\columnwidth}
\setlength{\tabcolsep}{1pt}
\renewcommand{\arraystretch}{-1} % Default value: 1

\begin{tabular}{cc}
\hspace{-0.32in}
\includegraphics[width=\w]{LaTeX/noisy_reference/ref_exp2.pdf}&
\hspace{-0.30in}
\includegraphics[width=\w]{LaTeX/noisy_reference/deg_exp2.pdf} &
\hspace{-0.3in}\includegraphics[width=\w]{LaTeX/noisy_reference/ref1_exp2.pdf} & 
\hspace{-0.3in}
\includegraphics[width=\w]{LaTeX/noisy_reference/deg1_exp2.pdf} \\
%

\begin{minipage}{\w}\centering
% \begin{spacing}{0.9}
\centering
{Reference recs.}
% \end{spacing}
\end{minipage} &

\begin{minipage}{\w}\centering
% \begin{spacing}{0.9}
\centering
{Test recs.}
% \end{spacing}
\end{minipage} &

\end{tabular}
\vspace{-1ex}
\caption{\textbf{Effect of Noise (2)}: \emph{Top Row}: original reference and test signals; \emph{Bottom Row}: same band-limited white noise added to both signals. \PESQ\ score increases by upto 0.2 points.}
\label{ref_deg_both_noise_added}
\vspace{-2ex}
\end{figure}

==> LaTeX/tables/ref_noise_added.tex <==
\begin{figure}[t!]
\vspace{-1.\baselineskip}
\centering
\setlength{\w}{0.33\columnwidth}
\setlength{\tabcolsep}{0pt}
\begin{tabular}{ccc}
\hspace{-0.2in}
\includegraphics[width=\w]{LaTeX/noisy_reference/ref_exp1.pdf}&
\hspace{-0.2in}
\includegraphics[width=\w]{LaTeX/noisy_reference/deg_exp1.pdf} &
\hspace{-0.2in}
\includegraphics[width=\w]{LaTeX/noisy_reference/ref1_exp1.pdf} \\
%
\begin{minipage}{\w}\centering
% \begin{spacing}{0.9}
\centering
{Reference rec.}
% \end{spacing}
\end{minipage} &
%
\begin{minipage}{\w}\centering
\centering
{Test rec.} 
\end{minipage} &
%
\begin{minipage}{\w}\centering
\vspace{0pt}
\centering
% \begin{spacing}{0.9}
{Ref. rec. + white band-limited noise}
% \end{spacing}
\end{minipage}
%
\end{tabular}
\vspace{-1.5ex}
\caption{\textbf{Effect of Noise (1)}: Band-limited white noise added to a reference recording. \PESQ\ score increases by upto 0.1 points.}
\label{ref_noise_added}
\vspace{-1.0ex}
%\vspace{-0.3in}
\end{figure}

==> LaTeX/tables/scenario3_test.tex <==
\begin{table}[t!]
\vspace{-0\baselineskip}
\centering
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3pt}
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c c c c c c c c c c c}
 \toprule
  \multirow{1}{*}{\bf Type} 
  %& \multicolumn{11}{c}{\bf Objective Metrics} \\
 %\cmidrule(lr){2-12} 
 &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQAPP & \bf NISQA  & \bf DNSMOS & \bf NORESQA  & \bf MOS \\
%  &\bf PESQ$\uparrow$ &\bf VISQOL$\uparrow$ &\bf DPAM$\downarrow$ &\bf CDPAM$\downarrow$ &\bf L1$\downarrow$ &\bf L2$\downarrow$ &\bf M.STFT$\downarrow$ & \bf SQAPP$\uparrow$ & \bf NISQA$\uparrow$  & \bf DNSMOS$\uparrow$ & \bf NORESQA$\downarrow$  & \bf MOS$\uparrow$ \\ 
 &\bf $\uparrow$ &\bf $\uparrow$ &\bf $\downarrow$ &\bf $\downarrow$ &\bf $\downarrow$ &\bf $\downarrow$ &\bf $\downarrow$ & \bf $\uparrow$ & \bf $\uparrow$  & \bf $\uparrow$ & \bf $\downarrow$  & \bf \uparrow$ \\
 \cmidrule(lr){1-13}
 
 {\bf VCTK Model} 
 & 3.13 & 4.18 & 1.35 & 0.07 & 0.30 & 2.14 & 0.07 & 3.76 & 4.65 & 3.55 & 10.53 & 4.10$\pm$0.05 \\
  \hline
 {\bf DAPS Model} 
 & 2.16 & 3.60 & 2.77 & 0.21 & 2.24 & 20.42 & 0.14 & 4.06 & 4.90 & 3.64 & 9.57 & 4.33$\pm$0.04\\
 {\bf \hspace{1mm} EQ Matching} 
 & 2.32 & 3.68 & 2.73  & 0.22 & 2.00 & 25.99 & 0.13 & 3.96 & 4.89 & 3.61 & 10.32 & 4.05$\pm$0.04 \\
 {\bf \hspace{1mm} Breath removal} 
 & 2.65 & 4.18 & 2.67 & 0.13 & 1.95 & 25.97 & 0.12 & 3.84 & 4.84 & 3.63 &  10.29 & 4.11$\pm$0.05\\
 {\bf \hspace{1mm} Energy norm} \\
 {\bf \hspace{3mm} itr0} 
 & 2.60 & 4.17 & 2.68  & 0.14 & 1.92 & 24.85  & 0.13 & 3.87 & 4.77 & 3.56 & 10.09 & 4.07$\pm$0.05\\
 {\bf \hspace{3mm} itr200} 
 & 2.54 & 4.17 & 2.69  & 0.14 & 1.92 & 24.83 & 0.14 & 3.94 & 4.78 & 3.55 & 10.07 & 4.04$\pm$0.05 \\
 {\bf \hspace{3mm} itr1000}
 & 2.54 & 4.17 & 2.69  & 0.15 & 1.91 & 24.77 & 0.14 & 3.95 & 4.78 &  3.55 &  10.07 & 3.95$\pm$0.05\\
 {\bf \hspace{1mm} Orig. Phase}
 & 3.24 & 4.44 & 1.21 & 0.05 & 0.21 & 0.25 & 0.13 & 3.97 & 4.78 & 3.60 &  10.35 & 4.09$\pm$0.05\\
 \bottomrule
\end{tabular}
}
% \vspace{-0.1in}
\caption{\textbf{Scenario 3}: Objective and subjective measures across various pre-processing stages when recordings from DAPS trained SE model are matched to the VCTK trained SE model.}
\vspace{-0.2in}
\label{pipeline}
\end{table}

==> LaTeX/texts/00-abstract.tex <==
\begin{abstract}
  
  Many audio processing tasks require perceptual assessment. 
  %
  However, the time and expense of obtaining ``gold standard'' human judgments limit the availability of such data. 
  %
  Therefore, objective metrics are necessary for many tasks that cannot incorporate a human in the loop.
  %
  Most applications incorporate full reference or other similarity-based metrics that depend on a clean reference.
  %
  Researchers have relied on such metrics to evaluate and compare various proposed methods, often concluding that small, measured differences imply one is 
  more effective than another.
  %
  In this paper, we demonstrate that objective similarity metrics can fail to correlate with human judgments of quality in several practical scenarios.
  %
  Moreover, for those scenarios, we compare full-reference metrics with no-reference metrics and show that the latter correlates better with human judgements. 
  %
  We conclude therefore that similarity provides only a weak proxy for audio quality.
  
\end{abstract}

  %\eg, \PESQ~\cite{rix2001perceptual}.
  %
  %However, due to the strict requirement of an explicit reference, no-reference metrics are attracting much attention. However, these methods were also found to generalise poorly to unseen noises.
  %
  %Therefore, due to their high familiarity, similarity metrics like PESQ have been the common go to approaches for objective quality assessment.
  %
  %In recent years, non-intrusive methods have attracted much attention since these don't need an explicit reference. However, these methods were also found to generalise poorly to unseen noises. Hence, similarity metrics like PESQ have been the go to objective metric in a lot of fields.
  %
  % twhere the ground truth clean references are not available.
  % Full-reference objective similarity metrics are used as a reliable proxy for absolute audio quality in lieu of human subjective ratings that are time consuming and need to be repeated many times.
  % Quality and Similarity/distance metrics are synonymously used as a proxy for estimating audio quality in the absence of subjective ratings. 
  %
    %The perceptual task of speech quality assessment (SQA) is a challenging task for machines to do. 
    %  This paper is intended both to illustrate and propagate the message that similarity metrics are only a weak proxy for audio quality. 
  %and also that existing no-reference metrics reflect absolute quality better than similarity metrics.
  %and should not be blindly used and trusted. It is also meant to encourage using no-reference (distance) metrics 
  
  %that the two may show different trends, depending on the context of usage. 
  %We take an example of a very well known existing similarity/distance metric (PESQ) and show practical scenarios where show its shortcomings. 
  %We provide guidance to researchers on where similarity metrics can/cannot be a reliable measure of quality and can be used as an evaluation tool. 
  %
  %Subsequently, we also show examples where PESQ fails as a quality metric showing un-naturally large distance even when the recordings show imperceptible differences. PESQ matching happens only under un-realistic conditions where we assume access to the ground truth magnitude and phase spectrum.


==> LaTeX/texts/01-intro.tex <==
\section{Introduction}

Speech quality assessment (SQA) plays a critical role in a range of audio and speech applications, including telephony, VoIP, hearing aids, automatic speech recognition, and speech enhancement. The ``gold standard'' for SQA involves human listening tests. However, these subjective evaluations are time consuming and expensive, as they require a human in the loop and often need to be repeated many times for every recording.
%
Thus automatic (objective) SQA methods are often more practical, and roughly fall into two categories -- whether or not they rely on a reference recording. 

\emph{Full-reference} metrics are also known as \emph{intrusive} or \emph{similarity} metrics (\eg\ \PESQ~\cite{rix2001perceptual}, \POLQA~\cite{beerends2013perceptual}, \VISQOL~\cite{hines2015visqol}, \DPAM~\cite{manocha2020differentiable}, \CDPAM~\cite{manocha2021cdpam} and others~\cite{patton2016automos,fu2019metricgan,yu2021metricnet}).
%
These metrics require a clean reference to which a corrupted signal can be compared as the basis for a quality rating; thus they cannot be applied in scenarios where the paired clean reference is unavailable. Moreover, full-reference methods are sensitive to perceptually invariant transformations~\cite{manjunath2009limitations,hines2013robustness}.

On the other hand, \emph{no-reference} metrics, also called \emph{non-intrusive}~\cite{loizou2011speech} metrics, (\eg\ \DNSMOS~\cite{reddy2020dnsmos}, \NISQA~\cite{mittag2021nisqa}, \SQAPP~\cite{Manocha:2022:SNS} and others~\cite{fu2018quality,andersen2018nonintrusive,lo2019mosnet,gamper2019intrusive,zhang2021end}) are designed to output a rating on an absolute scale, without access to a clean reference. 
However, these metrics: (i)~fail to generalize to unseen perturbations; (ii)~depend on an implicit clean reference that can be highly varying~\cite{manocha2021noresqa}, and (iii)~contain substantial label noise from human annotations~\cite{reddy2020dnsmos}.
%
To address a few concerns, researchers proposed using non-matching references \NORESQA~\cite{manocha2021noresqa} instead to increase robustness. However, it relies on SNR and Si-SDR that may not directly correlate with quality.

Researchers more commonly rely on full-reference metrics as a proxy for audio quality, because these frameworks have been around much longer~-- consider, \eg\ SNR~-- and they are more familiar.
%
Among full-reference metrics, one of the most impactful is \PESQ~\cite{rix2001perceptual}. Introduced more than two decades ago for telephony applications, it remains useful as a reliable proxy for subjective audio quality evaluations across fields including enhancement~\cite{su2020hifi,manocha2020differentiable,manocha2021cdpam,manocha2021noresqa,defossez2020real,zezario2021deep,Su:2021:HSS}, vocoders~\cite{cernak2005evaluation}, and transmission codecs~\cite{beerends2004measurement,paglierani2007uncertainty}. \PESQ\ models human auditory perception and correlates well with subjective listening tests~\cite{reddy2020dnsmos,fu2018end}. 
%
\PESQ\ labels have also been leveraged for training \emph{differentiable} quality metrics~\cite{fu2018quality,fu2019metricgan,xu2021deep}. 

There are many challenges in performing subjective tests, including the observation that ratings from different listening tasks cannot be compared~\cite{cooper2021generalization}.
%
Therefore, researchers rely on objective metrics like \PESQ\ for comparing the effectiveness of various methods, sometimes reporting small gains ($\sim$0.1 \PESQ).
%
However, \PESQ\ has acknowledged shortcomings~\cite{manjunath2009limitations,hines2013robustness}, and may not be reliable to detect subtle differences~\cite{manocha2020differentiable}.
%
Researchers have explored ways to ameliorate such shortcomings and improve robustness of these objective metrics~\cite{beerends2013perceptual,manocha2020differentiable}. 

This paper investigates the inherent limitations of the conventional formulation of similarity metrics, with the goal of informing future SQA research.
%
We describe three scenarios wherein we empirically evaluate seven similarity metrics (L1, L2, Multi-resolution STFT, \PESQ, \VISQOL, \DPAM\ and \CDPAM), and show that these contrast with subjective quality judgments. 
%
Overall, we find that: i)~similarity metrics may not respect the multi-modality of audio quality where recordings under different environments may be rated as equal quality; (ii)~a mismatch in the training and evaluation datasets may cause objective ratings to differ from subjective ratings (\eg\ speech enhancement); and (iii)~similarity metrics emphasize imperceptible differences, suggesting that these metrics fail for recordings that come from a completely different distribution but sound perceptually indistinguishable.
%
Additionally, we also show specific examples (\eg\ high-pass filtering, comparing cross-perturbations etc.) where similarity metrics contrast with subjective judgments. 
%
Moreover, on those same scenarios, we also evaluate four no-reference metrics (\DNSMOS, \NISQA, \SQAPP\ and \NORESQA) and show that these do not show the same shortcomings as similarity metrics. 
%
% mismatch in train and testt datasets, as well as these metrics just also being another types of sample level differences
%
These findings help in understanding the weaknesses of similarity metrics (\eg\ \PESQ), and help inform researchers on how best to use them across various tasks as a proxy for subjective audio quality judgments. 
%
% AF: I think the previous sentence is sufficient and the following sentence is too much.
%This paper is intended to illustrate the message that \PESQ\ (and other similarity metrics) are only a weak proxy for audio quality. 
%
All listening examples are available here:
\\{\footnotesize\tt\narrowstyle \href{https://percepaudio.cs.princeton.edu/Manocha22_QuaSim}{https://percepaudio.cs.princeton.edu/Manocha22\_QuaSim}}
%the general differences between similarity and quality metrics, as well as outline the guidelines where each can be used 'correctly' as an objective prediction for absolute audio quality.



% While we know that PESQ has its shortcomings, and bias of male over female ratings. 

%as well as ratings from 
%Moreover, given their high familiarity with similarity metrics like \PESQ, various researchers only report objective scores, with gains as low as 0.1 \PESQ\ score. 
% 
%This may be because subjective listener ratings are difficult to conduct, and moreover, ratings from two listening tasks cannot be compared~\cite{cooper2021generalization} since the ratings depend on the raters, the stimuli and the systems being evaluated.
%This is also suitable because listening test ratings typically depend on the listeners, stimuli and the ranges of systems being evaluated, and hence ratings from two listening tasks cannot be compared~\cite{cooper2021generalization}.
%


%While improving \PESQ\ (or other objective metric) is obvious and non-questionable, in this work we investigate the inherent challenges of the conventional formulation of similarity metrics using several scenarios where these metrics contrast with subjective quality. 
%
%At the same time, we also note no-reference metrics do not show the same drawbacks when evaluated in those scenarios.

%Our analysis stems from an observation that the \PESQ\ score (compared across the VCTK~\cite{valentini2017noisy} validation set) for a speech enhancement model that was trained on VCTK training set itself was higher than a model trained on another (DAPS~\cite{mysore2014can}) dataset, even though subjective listening suggests otherwise. Surprisingly, we found the same issue across all other similarity metrics we tested (L1, L2, Multi-resolution STFT, \VISQOL, \DPAM\ and \CDPAM). As we dug deeper, we also observed a similar trend across a newly released large dataset for speech enhancement (DDS)~\cite{li2021dds}. Overall, in this paper we empirically evaluate similarity metrics and show several scenarios where they fail, and also compare it to no-reference metrics (\DNSMOS, \NISQA, \SQAPP, \NORESQA) and show that these do not show the same shortcomings. 

==> LaTeX/texts/02-background.tex <==
\section{Related Work}
\label{sec:format}

\subsection{Full-reference and no-reference metrics}

Full-reference measures includes methods like \PESQ~\cite{rix2001perceptual}, \POLQA~\cite{beerends2013perceptual}, \VISQOL~\cite{hines2015visqol}, \DPAM~\cite{manocha2020differentiable} and \CDPAM~\cite{manocha2021cdpam}. Although quite useful, they suffer from two critical drawbacks. First, the requirement of a paired clean reference for SQA limits their applicability in scenarios where the paired clean reference is not available. Second, these methods are sensitive to perceptually invariant transformations~\cite{manjunath2009limitations,al2020correlation}.

In contrast, no-reference measures (\eg\ \DNSMOS~\cite{reddy2020dnsmos}, \NISQA~\cite{mittag2021nisqa}, \SQAPP~\cite{Manocha:2022:SNS}, and MetricNet~\cite{yu2021metricnet}) perform well in scenarios where a clean reference is not available. However, these metrics: (i)~fail to generalize to unseen perturbations; (ii)~depend on an implicit clean reference that can be highly varying~\cite{manocha2021noresqa}, and (iii)~contain substantial label noise from human annotations~\cite{reddy2020dnsmos}.
%
To address a few concerns, researchers proposed using non-matching references~\cite{manocha2021noresqa} instead to increase robustness. However, it relies on conventional metrics like SNR and SI-SDR that may not directly correlate with quality.

==> LaTeX/texts/05-analysis.tex <==
%\section{Analysis}

% \begin{enumerate}[leftmargin=0.33cm]
%     \setlength{\itemsep}{1pt}
%     \setlength{\parskip}{0pt}
%     \setlength{\parsep}{0pt}
    
%     \item Looking at the results in Tables~\ref{low_quality_sec4.2}, \ref{table_similarity_comparison}, and \ref{pipeline}, we see that similarity metrics fail to correlate with subjective quality, whereas distance metrics correlate well suggesting the usefulness of distance metrics in predicting absolute quality.
    
%     \item In Scenario 1 (Table~\ref{low_quality_sec4.2}), we showed that similarity metrics fail to provide equal scores for two reference recordings that both have equally good quality. However, we observe that distance metrics reflect the trend well.
    
%     \item In Table~\ref{tab:dds_environments}, we observe that all similarity metrics show high correlation with distance metrics and subjective listening scores when considered individually (DAPS and VCTK). This suggests that similarity metrics can be used to compare individually across each dataset. However, the estimate becomes incorrect when compared across datasets.
    
%     \item In Scenario 2 (Table~\ref{table_similarity_comparison}), we saw that a mismatch in training and evaluation clean datasets caused a variation between similarity metrics and subjective audio quality. 
%     % However, we also note that such a variation may still exist in similarity metrics even when there is no ove
%     %mismatch occurs (i.e., train and validation sets are different). 
%     The only way to possibly get rid of the discrepancy is to train and test models ``only'' on the same dataset(s). Moreover, results suggest that distance metrics can be used as proxy for subjective quality, and can reflect the trend well. Results also suggest that using a cleaner dataset (DAPS) for training an enhancement model leads to a qualitatively better model (as also confirmed by listening tests).
    
%     % training a model on a much cleaner dataset (DAPS) scores higher scores than the other dataset(VCTK). Focus on training on cleanest recordings
%     % \item In Scenario 1, we also note that we should also evaluate and compare PESQ scores on the clean (and unseen) test dataset.
    
%     \item In scenario 3 (Table~\ref{pipeline}), we showed that similarity metrics (e.g., \PESQ\ as well as other advanced metrics like \DPAM\ and \CDPAM) show that they emphasize low, sample-level differences and fail to reflect absolute quality even when the two recordings sound exactly the same, but do not come from the same distribution. 
    
    
    
%     % when there is no mismatch between clean references.
    
% %     MISC: DDS dataset: 
% %     - DAPS score is still lower than PESQ
% % - However the device, and direction change all show same trend when considered separately for each dataset. Good correlation across one dataset, but not when comparing 2 diff. datasets (Tables~\ref{device} and~\ref{positions})
% % - Adding noise to both recordings, bumps up PESQ scores, so PESQ algorithm may also try to match noise when the reference recording has noise, so in that case - the similarity with a clean test recording will be lower. 

%     %Three arguments
% %1. diff reference, same test, same quality, different distance
% %2. diff test, same reference, same quality, different distance
% %3. trying to match dataset => difficult or near impossible 
% \end{enumerate}

==> temp <==
\begin{table}[t!]
% \vspace{-1\baselineskip}
\centering
\resizebox{\columnwidth}{!}{
 \begin{tabular}{l c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multicolumn{3}{c}{\bf DAPS~\cite{jin2017voco}} & \multicolumn{3}{c}{\bf VCTK~\cite{su2019perceptually}} & \multicolumn{3}{c}{\bf Valset Clean~\cite{su2019perceptually}}\\
 \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10}
 &\bf PESQ & \bf NISQA & \bf SQUAPP & \bf PESQ & \bf NISQA & \bf SQUAPP &\bf PESQ & \bf NISQA & \bf SQUAPP\\
 \cmidrule(lr){1-10}
 
  {\bf Male} 
 & 2.49 & 4.95 & 38.61 & 3.22 & 4.64 & 38.05 & - & 4.65 & 35.99 \\
 {\bf Female} 
 & 1.85 & 4.75 & 37.86 & 3.05 & 4.55 & 37.25 & - & 4.66 & 35.97 \\
 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{M (F) Male and Female Scores} 
\label{tab:mos_1}
\end{table}


\begin{table*}[t!]
% \vspace{-1\baselineskip}
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c c c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multicolumn{10}{c}{\bf DAPS~\cite{jin2017voco}} & \multicolumn{10}{c}{\bf VCTK~\cite{su2019perceptually}} \\
 \cmidrule(lr){2-11} \cmidrule(lr){12-21} 
 &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS \\
 \cmidrule(lr){1-21}
 
  {\bf iPad} 
 & - & 4.679 & 35.623  & - & 4.13 & 33.837  \\
 {\bf Marantz} 
 & 1.551 & 2.892 & 31.861 & 1.701 & 2.813 & 31.373  \\
 {\bf Uber} 
 & 1.332 & 2.375 & 30.202 & 1.479 & 2.364 & 30.072 \\

 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{DDS Dataset - devices} 
\label{devices}
\end{table*}


\begin{table*}[t!]
% \vspace{-1\baselineskip}
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{l c c c c c c c c c c c c c c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multicolumn{10}{c}{\bf DAPS~\cite{jin2017voco}} & \multicolumn{10}{c}{\bf VCTK~\cite{su2019perceptually}} \\
 \cmidrule(lr){2-11} \cmidrule(lr){12-21} 
 &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS &\bf PESQ &\bf VISQOL &\bf DPAM &\bf CDPAM &\bf L1 &\bf L2 &\bf M.STFT & \bf SQUAPP & \bf NISQA  & \bf DNSMOS \\
 \cmidrule(lr){1-21}
 
  {\bf ch1} 
 & - & 4.679 & 35.623  & - & 4.13 & 33.837  \\
 {\bf ch2} 
 & 1.551 & 2.892 & 31.861 & 1.701 & 2.813 & 31.373  \\
 {\bf ch3} 
 & 1.332 & 2.375 & 30.202 & 1.479 & 2.364 & 30.072 \\
 {\bf ch4} 
 & 1.803 & 3.005 & 32.929 & 1.938 & 2.842 & 32.274 \\
 {\bf ch5} 
 & 1.568 & 2.707 & 32.023 & 1.701 & 2.641 & 31.499 \\
 {\bf ch6}
 & 1.594 & 2.704 & 31.596 & 1.723 & 2.649 & 30.955 \\

 \bottomrule
\end{tabular}
}
%\vspace{-0.1in}
\caption{DDS Dataset - Positions} 
\label{positions}
\end{table*}
